The Explicit Construction of Orders on Surfaces

We implement a noncommutative analogue of the well-known commutative cyclic covering trick and implement it to explicitly construct a vast collection of numerically Calabi-Yau orders, noncommutative analogues of surfaces of Kodaira dimension 0. We construct maximal orders, noncommutative analogues of normal schemes, on rational surfaces and ruled surfaces. We also use Ogg-Shafarevich theory to construct Azumaya algebras and, more generally, maximal orders on elliptically fibred surfaces.

==> c4.tex <==
Let $\rho\colon Z\to C$ be a fibration and $C'\to C$ a $2\colon 1$ cyclic Galois cover:
$$
\xymatrix{
 Y \ar[r]^\pi \ar[d]^p & Z \ar[d]^\rho\\
C' \ar[r]        & C
}
$$
Let $\s$ be the covering involution of $\pi$ and set $A\assign\oy\oplus\ls$. We then have a morphism of quasi-schemes
%
\begin{eqnarray*}
f\colon A & \to & C'\\ 
\end{eqnarray*}
%
given by
%
\begin{eqnarray*}
f^*\colon\tmop{Mod}C' & \to & \tmop{Mod}A\\
M                     & \mapsto & p^*(M)\otimes_{\oy}A\\
%
f_*\colon \tmop{Mod}A & \to & \tmop{Mod}C'\\
N                     & \mapsto & p_*N
\end{eqnarray*}
these are adjoint, $f$ is a flat morphism of quasi-schemes, etc...
% 
% 
\begin{definition}
A curve on $A$ is a 1-pure module $M\in\tmop{Mod}A$ which is a quotient of $A$. We call $M$ a curve of genus one if $h^0(M)=h^1(M)=1$. We call
% 
\begin{eqnarray*}
 f\colon A & \to & C'
\end{eqnarray*}
a genus 1 fibration if $f^*(\os_{C',p})$ is a genus one curve on $A$, for almost all $p\in C'$.
\end{definition}

We also give here a preliminary definition of what a section of $f$ should be
% 
\begin{definition}
A section of $f\colon A \to C'$ is a morphism of quasi-schemes $s\colon C' \to A$ such that $fs\colon C'\to C'$ is the identity on $C'$. That is, two functors
% 
\begin{eqnarray*}
s^*\colon \tmop{Mod}A & \to & \tmop{Mod}C'\\
s_*\colon\tmop{Mod}C' & \to & \tmop{Mod}A\\
\end{eqnarray*}
% 
such that $f_*s_*$ and $s^*f^*$ are both the identity on $\tmop{Mod}C'$.
\end{definition}


Now I claim that the following is a sufficient condition for $f$ to possess a section: $p$ has a section $d\colon C'\to Y$ and $A_D\assign A\otimes\os_D$ possesses a sheaf of left ideal $I$ such that $A_D/I\simeq\os_D$.

OTHERWISE KNOWN AS
% 
% 
\begin{proposition}
Let $A$ be constructed as above and always with fibration $f\colon A \to C'$. Let $p$ have a section $d\colon C'\to Y$ with $D\assign\tmop{im}d$. If $A_D$ has an ideal sheaf $I\hookrightarrow A_D$ such that $A_D/I\simeq\os_D$, then $f$ possesses a section.
% 
% 

\begin{proof}
% 
Firstly, in this case, $A_D\simeq \od \oplus \os_{D\s} \oplus \ldots \os_{D\s}^{n-1}$. Then I claim that $A_D/I$ is an $(A_D-A_D)$-bimodule.
We define the section $s\colon C'\to A$ as follows
% 
\begin{eqnarray*}
 s^*\colon \tmop{Mod}A & \to & \tmop{Mod}C'\\
N                      & \mapsto & d^*(N\otimes_A A_D/I)\\
s_*\colon\tmop{Mod}C' & \to & \tmop{Mod}A\\
M                     & \mapsto & d_*(M)\otimes_{\oy} A\otimes A_D/I
\end{eqnarray*}
Now show $s^*,s_*$ are adjoint and that $f_*s_*=s^*f^*=\tmop{id}_{\tmop{Mod}C'}$.
% 
% 
\begin{eqnarray*}
\tmop{Hom}_C(s^*N,M) & \simeq & \tmop{Hom}_C(d^*(N\otimes_A A_D/I),M)\\
                     & \simeq & \tmop{Hom}_Y(N\otimes_A A_D/I,d_*M)\\
                     & \simeq & \tmop{Hom}_A(N\otimes_A A_D/I \otimes_{\os_D} A,d_*M\otimes_{\os_D} A)\\
                     & \simeq & \tmop{Hom}_A(N\otimes_A A_D/I \otimes_{\os_D} A\otimes_A A_D/I,d_*M\otimes_{\os_D} A\otimes_A A_D/I)\\
                     & \simeq & \tmop{Hom}_A(N\otimes_A A_D/I,s_*M)\\
                     & \simeq & \tmop{Hom}_A(N,s_*M)\\
\end{eqnarray*}
% 
shows adjointness. Now
% 
\begin{eqnarray*}
 f_*s_*M & = & p_*((d_*M)\otimes_{\oy} A\otimes_A A_D/I)\\
         & = & p_* d_*M\\
         & = & M\\
s^*f^*M  & = & s^*(p^*(M)\otimes_{\oy} A) \\
         & = & d^*(p^*(M)\otimes_{\oy} A \otimes_A A_D/I)\\
         & = & d^*(p^*(M))
\end{eqnarray*}
I think the whole point is that 
% 
% 
\begin{eqnarray*}
 \tmop{Mod}D\longrightarrowlim^{-\otimes_{\oy}A\otimes_A A_D/I}\tmop{Mod}A\longrightarrowlim^{\tmop{forgetful}}\tmop{Mod}D
\end{eqnarray*}


is the identity.
\end{proof}

\end{proposition}

In general,
% 
\begin{eqnarray*}
 A\otimes\od & \simeq \od \oplus M_\s \oplus \ldots \oplus M_s^{n-1}
\end{eqnarray*}
% 
for some degree $0$ line bundle $M$ on $D$. If $M\not\simeq\od$, then $\od$ cannot be given the structure of an $A\otimes\od$-quotient since $\tmop{Hom}(M,\od)=0$.

To give $\od$ an  $A\otimes\od$-module structure we are required to give a morphism $L\otimes\s^*\od\longrightarrow\od$ aka $\psi\colon M\otimes\s^*\od\longrightarrow\od$ such that
% 
$$
\xymatrix{
M_\s \otimes M_\s \otimes \od \ar[r]^{1 \otimes \psi} \ar[d]^{\phi \otimes 1} & M_\s \otimes \od \ar[d]^\psi\\
% 
\od \otimes \od              \ar[r]^\sim                        & \od
}
$$
% 
Here $\phi\colon M_\s^2\longrightarrowlim^{\sim} \od$ is the overlap condition, generically multiplication by some $\alpha \in k(D/G)$.

Assuming $M \simeq \od$, then $\tmop{Hom}(M,\od)=k$ and the possible $\psi$ are of the form $\psi\colon M\otimes\s^*\od=\beta\od$, where $\beta^n=\alpha$ OR are given by multiplication by $\beta$, where $\beta^n=\alpha$.


